Scalable computational kernels for mortar finite element methods

Targeting simulations on parallel hardware architectures, this paper presents computational kernels for efficient computations in mortar finite element methods. Mortar methods enable a variationally consistent imposition of coupling conditions at high accuracy, but come with considerable numerical effort and cost for the evaluation of the mortar integrals to compute the coupling operators. In this paper, we identify bottlenecks in parallel data layout and domain decomposition that hinder an efficient evaluation of the mortar integrals. We then propose a set of computational strategies to restore optimal parallel communication and scalability for the core kernels devoted to the evaluation of mortar terms. We exemplarily study the proposed algorithmic components in the context of three-dimensional large-deformation contact mechanics, both for cases with fixed and dynamically varying interface topology, yet these concepts can naturally and easily be transferred to other mortar applications, e.g. classical meshtying problems. To restore parallel scalability, we employ overlapping domain decompositions of the interface discretization independent from the underlying volumes and then tackle parallel communication for the mortar evaluation by a geometrically motivated reduction of ghosting data. Using three-dimensional contact examples, we demonstrate strong and weak scalability of the proposed algorithms up to 480 parallel processes as well as study and discuss improvements in parallel communication related to mortar finite element methods. For the first time, dynamic load balancing is applied to mortar contact problems with evolving contact zones, such that the computational work is well balanced among all parallel processors independent of the current state of the simulation.

==> data/cyl_viz/o/cyl_viz_Dynamic_binning_proximityYes_sizeDDTol-1-03_maxImbalance-1-8_minEleProc-0_mpi024_owner_colorbar.tex <==
%% This file was created with pvutils
%% Use the following includes in the LaTeX header:
%\usepackage{tikz}
%\usepackage{pgfplots}
%% Optional:
%\pgfplotsset{compat=1.16}
%{\normalsize% Sometimes in figure environments a smaller font is selected -> uncomment this to activate the default font size
\begin{tikzpicture}
% The -0.2pt here are needed, so the immage is really placed at the origin.
\node[anchor=south west,inner sep=-0.2pt] (image) at (0,0) {\includegraphics[scale=0.24]{data/cyl_viz/o/cyl_viz_Dynamic_binning_proximityYes_sizeDDTol-1-03_maxImbalance-1-8_minEleProc-0_mpi024_owner_colorbar.png}};
\begin{axis}[
scale only axis,
scaled x ticks=false,
scaled y ticks=false,
at={(0.245533333333cm,1.1938cm)},
tick label style={font=\footnotesize},
title=Owner,
xticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
yticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
ymin=0.0,
ymax=23.0,
xmin=0.0,
xmax=23.0,
ytick=\empty,
height=0.211666666667cm,
width=4.4958cm,
xtick={0.0,23.0},
xtick pos=left,
xtick align=outside,
tick label style=below,
title style={yshift=-25pt,below},
]
\end{axis}
\end{tikzpicture}%
%}%

==> data/cyl_viz/o/cyl_viz_None_binning_proximityNo_sizeDDTol-1-03_maxImbalance-1-8_minEleProc-0_mpi024_owner_colorbar.tex <==
%% This file was created with pvutils
%% Use the following includes in the LaTeX header:
%\usepackage{tikz}
%\usepackage{pgfplots}
%% Optional:
%\pgfplotsset{compat=1.16}
%{\normalsize% Sometimes in figure environments a smaller font is selected -> uncomment this to activate the default font size
\begin{tikzpicture}
% The -0.2pt here are needed, so the immage is really placed at the origin.
\node[anchor=south west,inner sep=-0.2pt] (image) at (0,0) {\includegraphics[scale=0.24]{data/cyl_viz/o/cyl_viz_None_binning_proximityNo_sizeDDTol-1-03_maxImbalance-1-8_minEleProc-0_mpi024_owner_colorbar.png}};
\begin{axis}[
scale only axis,
scaled x ticks=false,
scaled y ticks=false,
at={(0.245533333333cm,1.1938cm)},
tick label style={font=\footnotesize},
title=Owner,
xticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
yticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
ymin=0.0,
ymax=23.0,
xmin=0.0,
xmax=23.0,
ytick=\empty,
height=0.211666666667cm,
width=4.4958cm,
xtick={0.0,23.0},
xtick pos=left,
xtick align=outside,
tick label style=below,
title style={yshift=-25pt,below},
]
\end{axis}
\end{tikzpicture}%
%}%

==> fig/basics_overlapping_dd/mesh.tex <==
% !TEX root = ../../contact_parallel_algos.tex

% grid lines
\foreach \x in {0,\h,...,\len}
  \draw [] (\x,0) -- (\x,\len);
\foreach \y in {0,\h,...,\len}
  \draw [] (0,\y) -- (\len,\y);


==> fig/contact_rolling_cyl_geometry.tex <==
% !TEX root = ../contact_parallel_algos.tex

\begin{tikzpicture}[tension=0.75,scale=1.0]

%\draw[help lines] (-2,-5) grid (10,5);

%% dimensions
\def\len{8}
\def\rad{2}
\def\height{1.5}
\def\tableWidth{2}
\def\cylWidth{1.8}
\def\mySin{0.707106781186548}
\def\myCos{0.707106781186548}

%%% coordinate axes
%\def\Ox{\Ax+1/4*\len*\cosFourtyTwo}
%\def\Oy{\Ay+\len*\sinFourtyTwo}
%\def\Xx{\Ox+1/2*\len*\cosSeven}
%\def\Xy{\Oy-1/2*\len*\sinSeven}
%\def\Yx{\Ox+1/2*\len*\cosFourtyTwo}
%\def\Yy{\Oy+1/2*\len*\sinFourtyTwo}
%\def\Zx{\Ox}
%\def\Zy{\Oy+1/2*\len}

%% some other definitions
\def\dist{0.1}
\def\auxlen{0.5}

%% domain

% clamping
%\fill [fill=black!30] (\Px,\Py+1/2*\len+\offsetDBC) -- (\Px,\Py-1/2*\len-\offsetDBC) -- (\Qx,\Qy-1/2*\len-\offsetDBC) -- (\Qx,\Qy+1/2*\len+\offsetDBC) -- cycle;

% white domain surfaces
%\fill [fill=white] (\Ax,\Ay+\len) -- (\Ax,\Ay) -- (\Cx,\Cy) -- (\Cx,\Cy+\len) -- cycle;
%\fill [fill=white] (\Ax,\Ay+\len) -- (\Fx,\Fy+\len) -- (\Dx,\Dy+\len) -- (\Cx,\Cy+\len) -- cycle;
%\fill [fill=white] (\Bx,\By-\thick) -- (\Cx,\Cy-\thick) -- (\Cx,\Cy+\thick);
%\draw [domainline] (\Ax,\Ay) -- (\Bx,\By) -- (\Cx,\Cy);

%% domain outlines
% visible lines of block
\draw [domainline] (0,0) rectangle (\len,\height);
\draw [domainline] (0,\height) -- (\tableWidth*\myCos,\tableWidth*\mySin+\height) -- (\tableWidth*\myCos+\len,\tableWidth*\mySin+\height) -- (\len,\height);
\draw [domainline] (\len,0) -- (\len+\tableWidth*\myCos,\tableWidth*\mySin) -- (\len+\tableWidth*\myCos,\tableWidth*\mySin+\height);

% hidden lines of block
\draw [hiddenline] (0,0) -- (\tableWidth*\myCos,\tableWidth*\mySin) -- (\tableWidth*\myCos+\len,\tableWidth*\mySin);
\draw [hiddenline] (\tableWidth*\myCos,\tableWidth*\mySin) -- (\tableWidth*\myCos,\tableWidth*\mySin+\height);

% visible lines of cylinder


% measurements
%\draw [measauxline] (\Ax,\Ay-\dist) -- (\Ax,\Ay-\dist-\auxlen);
%\draw [measauxline] (\Bx,\By-\dist) -- (\Bx,\By-\dist-\auxlen);
%\draw [measauxline] (\Cx,\Cy-\dist) -- (\Cx,\Cy-\dist-\auxlen);
%\draw [measauxline] (\Dx,\Dy-\dist) -- (\Dx,\Dy-\dist-\auxlen);
%\draw [measline] (\Ax,\Ay-\auxlen) -- (\Bx,\By-\auxlen);
%\draw [measline] (\Bx,\By-\auxlen) -- (\Cx,\Cy-\auxlen);
%\draw [measline] (\Cx,\Cy-\auxlen) -- (\Dx,\Dy-\auxlen);

%\draw [measauxline] (\Dx+1/2*\dist*\cosFourtyTwo,\Dy+1/2*\dist*\sinFourtyTwo) -- (\Dx+3/2*\dist*\cosFourtyTwo+1/2*\auxlen*\cosFourtyTwo,\Dy+3/2*\dist*\sinFourtyTwo+1/2*\auxlen*\sinFourtyTwo);
%\draw [measauxline] (\Dx+1/2*\dist*\cosFourtyTwo,\Dy+\len+1/2*\dist*\sinFourtyTwo) -- (\Dx+3/2*\dist*\cosFourtyTwo+1/2*\auxlen*\cosFourtyTwo,\Dy+\len+3/2*\dist*\sinFourtyTwo+1/2*\auxlen*\sinFourtyTwo);
%\draw [measline] (\Dx+1/2*\dist*\cosFourtyTwo+1/2*\auxlen*\cosFourtyTwo,\Dy+1/2*\auxlen*\sinFourtyTwo) -- (\Dx+1/2*\dist*\cosFourtyTwo+1/2*\auxlen*\cosFourtyTwo,\Dy+\len+1/2*\auxlen*\sinFourtyTwo);
%
%\node [below] at (\Ax+1/2*\len*\cosSeven,\Ay-\auxlen-1/2*\len*\sinSeven) {$\ell$};
%\node [below] at (\Bx+1/2*\len*\cosSeven,\By-\auxlen-1/2*\len*\sinSeven) {$\ell$};
%\node [below] at (\Cx+1/4*\len*\cosFourtyTwo,\Cy-\auxlen+1/4*\len*\sinFourtyTwo) {$\ell$};
%\node [right] at (\Dx+1/2*\dist*\cosFourtyTwo+1/2*\auxlen*\cosFourtyTwo,\Dy+1/2*\auxlen*\sinFourtyTwo+1/2*\len) {$\ell$};

% axes
%\draw [coordline] (\Ox,\Oy) -- (\Xx,\Xy);
%\draw [coordline] (\Ox,\Oy) -- (\Yx,\Yy);
%\draw [coordline] (\Ox,\Oy) -- (\Zx,\Zy);
%
%%\node [below] at (\Ox,\Oy) {O};
%\node [right] at (\Xx,\Xy) {$\xaxis$};
%\node [right] at (\Yx,\Yy) {$\yaxis$};
%\node [right] at (\Zx,\Zy) {$\zaxis$};

%%% annotations
%% naming of domains
% left
%\node at (\Ax+1/2*\len*\cosSeven+1/4*\len*\cosFourtyTwo,\Ay+1/2*\len*\sinSeven+1/4*\len*\sinFourtyTwo+3/2*\len) {$\Dom{1}$};
% right
%\node at (\Mx,\My) {$\Dom{2}$};
% interface
%\node [shift={(0,-\offsetInterface)},right] at (\Kx,\Ky) {$\CoupBound$};

\end{tikzpicture}

==> fig/cubes_interface_dd/cubes_viz_None_binning_mpi024_owner_3d.tex <==
%% This file was created with pvutils
%% Use the following includes in the LaTeX header:
%\usepackage{tikz}
%\usepackage{pgfplots}
%% Optional:
%\pgfplotsset{compat=1.16}
%{\normalsize% Sometimes in figure environments a smaller font is selected -> uncomment this to activate the default font size
\begin{tikzpicture}
% The -0.2pt here are needed, so the immage is really placed at the origin.
\node[anchor=south west,inner sep=-0.2pt] (image) at (0,0) {\includegraphics[scale=0.24]{fig/cubes_interface_dd/cubes_viz_None_binning_mpi024_owner_3d.png}};
\begin{axis}[
scale only axis,
scaled x ticks=false,
scaled y ticks=false,
at={(0.956733333333cm,3.9878cm)},
tick label style={font=\footnotesize},
title=Owner,
xticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
yticklabel={$\pgfmathprintnumber[precision=0]{\tick}$},
ymin=0.0,
ymax=23.0,
xmin=0.0,
xmax=23.0,
ytick=\empty,
height=0.169333333333cm,
width=2.8702cm,
xtick={0.0,23.0},
xtick pos=right,
xtick align=outside,
tick label style=above,
title style={yshift=10pt,above},
]
\end{axis}
\end{tikzpicture}%
%}%

==> fig/interface_storage/bins.tex <==
% !TEX root = ../../contact_parallel_algos.tex

\input{./fig/interface_storage/common_defines.tex}

% bins
\foreach \x in {0,1,...,\numXBins}
  \draw[thick,solid,\colorBins] (\masterLength/2 - \numXBins/2*\binSize + \x*\binSize + \xshiftBins,-\binSize+\gap/2) -- (\masterLength/2 - \numXBins/2*\binSize + \x*\binSize + \xshiftBins,\binSize+\gap/2);
\foreach \y in {-1,0,1}
    \draw[thick,solid,\colorBins] (\masterLength/2 - \numXBins/2*\binSize + \xshiftBins, \y*\binSize+\gap/2) -- (\masterLength/2 + \numXBins/2*\binSize + \xshiftBins, \y*\binSize+\gap/2);
  

==> fig/interface_storage/common_defines.tex <==
% !TEX root = ../../contact_parallel_algos.tex

% A set of common definitions used in all mesh sketches
\def\slaveLength{3.25cm} % horizontal width of slave domain
\def\masterLength{4.0cm} % horizontal width of master domain
\def\gap{0.6cm} % vertical width of gap
\def\xOffset{0.4cm} % horizontal indentation of top (slave) domain

\def\colorProcOne{red} % color for proc 0
\def\colorProcTwo{blue} % color for proc 1
\def\colorProcThree{green!40!black} % color for proc 2

\def\padding{0.7mm} % padding for coloring subdomains

\def\verticalShift{1.3mm} % vertical offset for overlapping master subdomains 

\def\h{0.25cm} % mesh size

\def\boxLeft{-0.65cm}
\def\boxBottom{-0.8cm}
\def\boxWidth{4.85cm} % width of surrounding dashed box
\def\boxHeight{2.2cm} % height of surrounding dashed box
\def\dist{0.1cm} % distance between two boxes


==> fig/interface_storage/master_defines.tex <==
% !TEX root = ../../contact_parallel_algos.tex

% Nodes for subdomains on master side
\node (mA) at (0,0) {};  % start of proc 0
\node (mB) at (1.5,0) {}; % end of proc 0
\node (mC) at (1.75,0) {}; % start of proc 1
\node (mD) at (3.0,0) {}; % end of proc 1
\node (mE) at (3.25,0) {}; % start of proc 2
\node (mF) at (4.0,0) {}; % end of proc2


==> fig/interface_storage/meshes.tex <==
% !TEX root = ../../contact_parallel_algos.tex

\input{./fig/interface_storage/common_defines.tex}

\draw[dotted, thick, rounded corners, fill=white, fill opacity=0.2, color=gray] (\boxLeft,\boxBottom) rectangle (\boxLeft+\boxWidth,\boxBottom+\boxHeight);

%% Master body with interface
\begin{scope}[xshift=0,yshift=0]

\foreach \y in {0,-0.25,...,-0.5}{
  \draw [gridline]  (0,\y) -- (\masterLength,\y);
}

\foreach \x in {0,0.25,...,4}{
  \node[draw,circle,inner sep=0.8pt,fill] at (\x,0) {};
  \draw [gridline] (\x,0) -- (\x,-0.65);
}

\node[left] at (0,0) {$\indexedMaster{\CoupBound}$};

\end{scope} % end of scope for slave body

%% Slave body with interface
\begin{scope}[xshift=\xOffset,yshift=\gap]

\foreach \y in {0,0.25,...,0.5}{
  \draw [gridline] (0,\y) -- (\slaveLength,\y);
}

\foreach \x in {0,0.25,...,3.25}{
  \node[draw,circle,inner sep=0.8pt,fill] at (\x,0) {};
  \draw [gridline] (\x,0) -- (\x,0.65);
}

\node[left] at (0,0) {$\indexedSlave{\CoupBound}$};
\end{scope}

%% Active contact interface
%\begin{scope}[xshift=\xOffset,yshift=1/2*\gap]
%
%\draw [domainline,color=gray] (0.0,0.0) -- (\slaveLength,0.0);
%\foreach \x in {0.0, 0.25,...,3.25}{
%  \node[draw,circle,color=gray,fill=gray,inner sep=0.8pt,fill] at (\x,0.0) {};
%}
%\end{scope}

% Nodes for found active set portions
\def\startOfActiveSet{\xOffset}
\node (aA) at (\startOfActiveSet,1/2*\gap) {}; 
\node (aB) at (\startOfActiveSet+2*\h,1/2*\gap) {}; 
\node (aC) at (\startOfActiveSet+3*\h,1/2*\gap) {}; 
\node (aD) at (\startOfActiveSet+5*\h,1/2*\gap) {};
\node (aE) at (\startOfActiveSet+8*\h,1/2*\gap) {}; 
\node (aF) at (\startOfActiveSet+9*\h,1/2*\gap) {};
\node (aG) at (\startOfActiveSet+11*\h,1/2*\gap) {};
\node (aH) at (\startOfActiveSet+\slaveLength,1/2*\gap) {};


==> fig/interface_storage/neighboring_bins.tex <==
% !TEX root = ../../contact_parallel_algos.tex

\begin{tikzpicture}

% load common definitions
\input{./fig/interface_storage/common_defines.tex}

\def\colorBins{orange} % color for bins
\def\binSize{0.59cm} % size of bins
\def\xshiftBins{0.0cm} % shift bins in x-direction
\def\numBinsPerDir{3} % number of bins in x-direction
\def\numXBins{7} % number of bins in x-direction

\begin{scope}[scale=1.1] % scope for entire picture

\draw[fill=red!10!white] (0,0) rectangle (\numBinsPerDir*\binSize,\numBinsPerDir*\binSize);
\draw[fill=green!10!white] (\binSize,\binSize) rectangle (2*\binSize,2*\binSize);

\foreach \binID in {0,1,...,\numBinsPerDir}{
  \draw[thick,solid,\colorBins] (\binID*\binSize,0) -- (\binID*\binSize,\numBinsPerDir*\binSize);
  \draw[thick,solid,\colorBins] (0,\binID*\binSize) -- (\numBinsPerDir*\binSize,\binID*\binSize);
}

\end{scope} % scope for entire picture

\end{tikzpicture}


==> fig/interface_storage/par_dist_color_legend.tex <==
% !TEX root = ../../contact_parallel_algos.tex

% Legend for process coloring and color for active set/found contact nearest neighbors

%\node at (0,3em) {found};
\node at (0,2em) {proc $0$};
\node at (0,1em) {proc $1$};
\node at (0,0em) {proc $2$};

\def\colorLeft{0.6cm}
\def\colorRight{0.9cm}

%% Found contact nearest neighbors
%\node (pColorFoundLeft) at (\colorLeft,3em) {};
%\node (pColorFoundRight) at (\colorRight,3em) {};
%\draw[thick,gray,fill=gray,fill opacity=0.2] \convexpath{pColorFoundLeft,pColorFoundRight}{\padding};

% Processes
\node (pColorOneLeft) at (\colorLeft,2em) {};
\node (pColorOneRight) at (\colorRight,2em) {};

\node (pColorTwoLeft) at (\colorLeft,1em) {};
\node (pColorTwoRight) at (\colorRight,1em) {};

\node (pColorThreeLeft) at (\colorLeft,0em) {};
\node (pColorThreeRight) at (\colorRight,0em) {};

\draw[thick,\colorProcOne,fill=\colorProcOne,fill opacity=0.2] \convexpath{pColorOneLeft,pColorOneRight}{\padding};
\draw[thick,\colorProcTwo,fill=\colorProcTwo,fill opacity=0.2] \convexpath{pColorTwoLeft,pColorTwoRight}{\padding};
\draw[thick,\colorProcThree,fill=\colorProcThree,fill opacity=0.2] \convexpath{pColorThreeLeft,pColorThreeRight}{\padding};


==> fig/interface_storage/slave_subdomains.tex <==
% !TEX root = ../../contact_parallel_algos.tex

% Nodes for subdomains on slave side
\node (sA) at (\xOffset,\gap) {}; 
\node (sB) at (\xOffset+0.5cm,\gap) {}; 
\node (sC) at (\xOffset+0.75cm,\gap) {}; 
\node (sD) at (\xOffset+2.0cm,\gap) {};
\node (sE) at (\xOffset+2.25cm,\gap) {}; 
\node (sF) at (\xOffset+3.25cm,\gap) {};

% draw slave interface subdomains
\draw[thick,\colorProcOne,fill=\colorProcOne,fill opacity=0.2] \convexpath{sA,sB}{\padding};
\draw[thick,\colorProcTwo,fill=\colorProcTwo,fill opacity=0.2] \convexpath{sC,sD}{\padding};
\draw[thick,\colorProcThree,fill=\colorProcThree,fill opacity=0.2] \convexpath{sE,sF}{\padding};


==> fig/problem.tex <==
% !TEX root = ../contact_parallel_algos.tex

\begin{tikzpicture}[tension=0.75,scale=1.0]

%\draw[help lines] (-2,-5) grid (10,5);

%% some coordinate definitions for domain boundaries
\def\Ax{2.0}
\def\Ay{-1.5}
\def\Bx{0.7}
\def\By{-1.2}
\def\Cx{0.0}
\def\Cy{0.0}
\def\Dx{0.9}
\def\Dy{1.3}
\def\Ex{2.1}
\def\Ey{1.0}
\def\Fx{2.5}
\def\Fy{1.0}
\def\Gx{4.2}
\def\Gy{1.4}
\def\Hx{5.0}
\def\Hy{0.0}
\def\Ix{3.5}
\def\Iy{-1.2}
\def\Jx{2.5}
\def\Jy{0.3}
\def\Kx{2.1}
\def\Ky{-0.7}

%% some coordinate definitions for annotations
% positioninig of \flu{\dom}
\def\Lx{1.2}
\def\Ly{0.0}
% positioning of \str{\dom}
\def\Mx{3.7}
\def\My{0.1}
% positioning of \flusub{\teo\trac}{\FSII}
\def\Nx{2.5}
\def\Ny{0.4}
% positioning of \strsub{\teo\trac}{\FSII}
\def\Ox{2.1}
\def\Oy{-0.7}

%% some other definitions
\def\offsetDomOne{5.9cm} % offset of fluid free body diagram
\def\offsetDomTwo{2.5cm} % offset of structure free body diagram
\def\boundlength{0.1} % length of boundary-conditioning-indicating lines
\def\tracx{0.05} % distance of traction vectors from interface in x-direction
\def\tracy{0.25} % distance between traction vectors in y-direction
\def\traclengthx{0.7} % length of traction vectors in x-direction
\def\traclengthy{0.4} % length of traction vectors in y-direction
\def\offsetInterface{0.3}

%% left: entire domain

%% domain lines
% left domain with index 1
\draw plot[smooth] coordinates{(\Ax,\Ay) (\Bx,\By) (\Cx,\Cy) (\Dx,\Dy) (\Ex,\Ey) (\Fx,\Fy)};
% right domain with index 2
\draw plot[smooth] coordinates{(\Fx,\Fy) (\Gx,\Gy) (\Hx,\Hy) (\Ix,\Iy) (\Ax,\Ay)};
% interface
\draw plot[smooth] coordinates{(\Fx,\Fy) (\Jx,\Jy) (\Kx,\Ky) (\Ax,\Ay)};
  
%% for debugging: Place letters for control nodes
%\node at (\Ax,\Ay) {A};
%\node at (\Bx,\By) {B};
%\node at (\Cx,\Cy) {C};
%\node at (\Dx,\Dy) {D};
%\node at (\Ex,\Ey) {E};
%\node at (\Fx,\Fy) {F};
%\node at (\Gx,\Gy) {G};
%\node at (\Hx,\Hy) {H};
%\node at (\Ix,\Iy) {I};%\node at (\Jx,\Jy) {J};
%\node at (\Kx,\Ky) {K};
%% end of debugging
  
\draw (\Cx-\boundlength,\Cy) -- (\Cx+\boundlength,\Cy);
\draw (\Hx-\boundlength,\Hy+0.2) -- (\Hx+\boundlength,\Hy+0.2);

%%% annotations
%% naming of domains
% left
\node at (\Lx,\Ly) {$\Dom{1}$};
% right
\node at (\Mx,\My) {$\Dom{2}$};
% interface
\node [shift={(0,-\offsetInterface)},right] at (\Kx,\Ky) {$\CoupBound$};
% Dirichlet boundary of domain #1
\node [above left] at (\Dx,\Dy) {$\indexedDom{\DBound}{1}$};
% Neumann boundary of domain #1
\node [below left] at (\Bx,\By) {$\indexedDom{\NBound}{1}$};
% Dirichlet boundary of domain #2
\node [above right] at (\Gx,\Gy) {$\indexedDom{\DBound}{2}$};
% Neumann boundary of domain #2
\node [below right] at (\Ix,\Iy) {$\indexedDom{\NBound}{2}$};



%%% right: free body diagram
%\begin{scope}[shift={(\offsetDomOne,0)}]
%  %% left domain #1)
%  % outer boundary
%  \draw plot[smooth] coordinates{(\Ax,\Ay) (\Bx,\By) (\Cx,\Cy) (\Dx,\Dy) (\Ex,\Ey) (\Fx,\Fy)};
%  % interface
%  \draw plot[smooth] coordinates{(\Fx,\Fy) (\Jx,\Jy) (\Kx,\Ky) (\Ax,\Ay)};
%  
%  %% right domain #2
%	% outer boundary
%  \draw [xshift=\offsetDomTwo] plot[smooth] coordinates{(\Fx,\Fy) (\Gx,\Gy) (\Hx,\Hy) (\Ix,\Iy) (\Ax,\Ay)};
%  % interface
%  \draw [xshift=\offsetDomTwo] plot[smooth] coordinates{(\Fx,\Fy) (\Jx,\Jy) (\Kx,\Ky) (\Ax,\Ay)};
%  
%  % tics for boundary subdivision
%  \draw (\Cx-\boundlength,\Cy) -- (\Cx+\boundlength,\Cy);
%  \draw [xshift=\offsetDomTwo] (\Hx-\boundlength,\Hy+0.2) -- (\Hx+\boundlength,\Hy+0.2);
%  
%  %%% interface traction vectors
%  % domain #1 (from top to bottom)
%  \draw [tractionarrow] (\Jx+2*\tracx,\Jy+\tracy) -- (\Jx+2*\tracx+\traclengthx,\Jy+\tracy-\traclengthy);
%  \draw [tractionarrow] (\Jx+\tracx,\Jy) -- (\Jx+\tracx+\traclengthx,\Jy-\traclengthy);
%  \draw [tractionarrow] (\Jx,\Jy-\tracy) -- (\Jx+\traclengthx,\Jy-\tracy-\traclengthy);
%  % domain #2 (from top to bottom)
%  \draw [xshift=\offsetDomTwo,tractionarrow] (\Kx,\Ky+\tracy) -- (\Kx-\traclengthx,\Ky+\tracy+\traclengthy);
%  \draw [xshift=\offsetDomTwo,tractionarrow] (\Kx-\tracx,\Ky) -- (\Kx-\tracx-\traclengthx,\Ky+\traclengthy);
%  \draw [xshift=\offsetDomTwo,tractionarrow] (\Kx-2*\tracx,\Ky-\tracy) -- (\Kx-2*\tracx-\traclengthx,\Ky-\tracy+\traclengthy);
%
%  %%% annotations
%  %% naming of domains
%  % domain #1
%  \node at (\Lx,\Ly) {$\Dom{1}$};
%  % domain #2
%  \node [xshift=\offsetDomTwo] at (\Mx,\My) {$\Dom{2}$};
%  % interface
%  \node [shift={(0,-\offsetInterface)},right] at (\Kx,\Ky) {$\CoupBound$}; % left: domain #1
%  \node [shift={(\offsetDomTwo,\offsetInterface)},left] at (\Jx,\Jy) {$\CoupBound$}; % right: domain #2
%  % Dirichlet boundary of domain #1
%  \node [above left] at (\Dx,\Dy) {$\indexedDom{\DBound}{1}$};
%  % Neumann boundary of domain #1
%  \node [below left] at (\Bx,\By) {$\indexedDom{\NBound}{1}$};
%  % Dirichlet boundary of domain #2
%  \node [xshift=\offsetDomTwo,above right] at (\Gx,\Gy) {$\indexedDom{\DBound}{2}$};
%  % Neumann boundary of domain #2
%  \node [xshift=\offsetDomTwo,below right] at (\Ix,\Iy) {$\indexedDom{\NBound}{2}$};
%  % interface traction onto domain #1
%  \node [above right] at (\Nx,\Ny+0.1) {$\indexedDom{\CoupInd{\teo\trac}}{1}$};
%  % interface traction onto domain #2
%  \node [xshift=\offsetDomTwo-\offsetInterface,below left] at (\Ox,\Oy-0.1) {$\indexedDom{\CoupInd{\teo\trac}}{2}$};
%\end{scope}

\end{tikzpicture}

==> fig/split_slave/split_slave_interface.tex <==
% !TEX root = ../../contact_parallel_algos.tex

\usetikzlibrary{fadings}

\begin{tikzpicture}[scale=1.5,font=\scriptsize]

\def\masterLength{6}
\def\masterHeigth{0.5}
\def\hx{0.25}

\def\slaveRadius{0.7}

% Master: grid with nodes
\begin{scope}[yshift=0]
% grid lines of master subdomain
\foreach \y in {0,-\hx,...,-\masterHeigth}{
  \draw [gridline,color=gray]  (0,\y) -- (\masterLength,\y);
}

% interface nodes of master
\foreach \x in {0,\hx,...,\masterLength}{
  \draw [gridline,color=gray] (\x,0) -- (\x,-\masterHeigth);
  \node[draw,circle,inner sep=0.8pt,color=gray,fill] at (\x,0) {};
}

% interior nodes of master subdomain
\foreach \x in {0,\hx,...,\masterLength}{
  \foreach \y in {-\hx,-\masterHeigth}{
    \node[draw,circle,inner sep=0.8pt,color=gray,fill=white] at (\x,\y) {};
  }
}

% annotation of master interface
\draw [color=gray] (-0.1, 0) .. controls (-0.3,0.2) and (-0.4,-0.2) .. (-0.6,0.0);
\node [left,color=gray] at (-0.6,0) {$\indexedMaster{\Bound}$};

\end{scope} % end of master

% Slave: grid with nodes
\begin{scope}[shift={(0.15*\masterLength,\slaveRadius+0.1)}]
% grid lines for slave subdomain
%\draw [gridline,color=gray] (0,0) circle (\slaveRadius);
\draw [gridline,color=gray] (0,0) circle (0.75*\slaveRadius);
\draw [gridline,color=gray] (0,0) circle (0.5*\slaveRadius);

% interior slave nodes
\foreach \i in {0,...,17} {
  \draw[gridline,color=gray] (\i*360/17:0.5*\slaveRadius) -- (\i*360/17:\slaveRadius);
  \foreach \r in {0.5,0.75}{
    \node[draw,circle,inner sep=0.8pt,color=gray,fill=white] at (\i*360/17:\r*\slaveRadius) {};
  }
}

% close slave nodes/elements
\draw[gridline, red] (10/17*360:\slaveRadius) arc[start angle=10/17*360, end angle=16/17*360, radius=\slaveRadius];
\foreach \i in {11,...,15} {
  \node[draw,circle,inner sep=0.8pt,fill,color=red] at (\i*360/17:\slaveRadius) {};
}

% non-close slave nodes/elements
\draw[gridline, blue] (-1/17*360:\slaveRadius) arc[start angle=-1/17*360, end angle=10/17*360, radius=\slaveRadius];
\foreach \i in {-1,...,10} {
  \node[draw,circle,inner sep=0.8pt,fill,color=blue] at (\i*360/17:\slaveRadius) {};
}

% annotation of slave interface
\draw [color=gray] (-\slaveRadius-0.1, 0) .. controls (-\slaveRadius-0.3,0.2) and (-\slaveRadius-0.4,-0.2) .. (-\slaveRadius-0.6,0.0);
\node [left,color=gray] at (-\slaveRadius-0.6,0) {$\indexedSlave{\Bound}$};

% horizontal line to mark vicinity to the master interface
\draw[very thick,dashed,color=green!30!black,path fading=west] (-\slaveRadius-0.7,-0.63*\slaveRadius) -- (-0.5,-0.63*\slaveRadius);
\draw[very thick,dashed,color=green!30!black] (-0.5,-0.63*\slaveRadius) -- (0.5,-0.63*\slaveRadius);
\draw[very thick,dashed,color=green!30!black,path fading=east] (0.5,-0.63*\slaveRadius) -- (\slaveRadius+0.7,-0.63*\slaveRadius);

\end{scope} % end of slave

% legend
\begin{scope}[shift={(0.2*\masterLength+2.5*\slaveRadius,2ex)}]

\def\dy{1.2ex}

\node[draw,circle,inner sep=0.8pt,color=gray,fill=white] at (0.0,4*\dy) {};
\node[draw,circle,inner sep=0.8pt,color=red,fill] at (0.0,3*\dy) {};
\draw[gridline,red] (-0.12,3*\dy) -- (0.12,3*\dy);
\node[draw,circle,inner sep=0.8pt,color=blue,fill] at (0.0,2*\dy) {};
\draw[gridline,blue] (-0.12,2*\dy) -- (0.12,2*\dy);
\node[draw,circle,inner sep=0.8pt,color=gray,fill] at (0.0,1*\dy) {};
\draw[very thick,dashed,color=green!30!black] (-0.3,0*\dy) -- (0.1,0*\dy);

\node[right=1ex] at (0.0,4*\dy) {interior nodes};
\node[right=1ex] at (0.0,3*\dy) {``close'' nodes/elements on~$\indexedSlave{\Bound}$};
\node[right=1ex] at (0.0,2*\dy) {``non-close'' nodes/elements on~$\indexedSlave{\Bound}$};
\node[right=1ex] at (0.0,1*\dy) {nodes on~$\indexedMaster{\Bound}$};
\node[right=1ex] at (0.0,0*\dy) {vicinity of~$\indexedMaster{\Bound}$};
\end{scope} % end of legend

\end{tikzpicture}


==> fig/tikz_defines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% author: Matthias Mayr %%
%% date: 12/2015         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This is the central place to define global tikz commands and styles to be used in every tikz picture.

% load some libraries
\usetikzlibrary{arrows.meta}
\usetikzlibrary{bending}
\usetikzlibrary{positioning}
%\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{snakes}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{calc}

% line styles
\tikzstyle{domainline}=[thick]
\tikzstyle{hiddenline}=[thick,dashed]
\tikzstyle{dbcline}=[thick]
\tikzstyle{tractionline}=[thick]
\tikzstyle{tractionarrow}=[thick,-{Latex}]
\tikzstyle{measline}=[thick, {Latex}-{Latex}]
\tikzstyle{measradius}=[thick, -{Latex}]
\tikzstyle{measauxline}=[thick]
\tikzstyle{coordsline}=[thick,{Latex[open,fill=white]}-{Latex[open,fill=white]}]
\tikzstyle{coordline}=[thick,-{Latex[open,fill=white]}]
\tikzstyle{symmetryline}=[very thick,dash pattern=on 10pt off 3pt on \the\pgflinewidth off 3pt]

% define my own colors
\tikzstyle{darkgreen}=[green!50!black]

% springs
\tikzstyle{springlineal}=[snake=zigzag,thick,line before snake=0.5cm,line after snake=0.5cm,segment length=6,segment amplitude=5,join=round]

% for algorithmic flow charts
%\tikzstyle{actionnode}=[rectangle,minimum width=30mm,thick,draw,fill=gray!70]
%\tikzstyle{decisionnode}=[diamond,aspect=3,minimum size=6mm,thick,draw,fill=gray!70]
%\tikzstyle{startendnode}=[rectangle,minimum size=6mm,thick,draw]
\tikzstyle{flowchartarrow}=[thick,-{Latex}]




